ASIL: Augmented Structural Information Learning for Deep Graph Clustering in Hyperbolic Space

Graph clustering is a longstanding topic in machine learning. Recently, deep methods have achieved results but still require predefined cluster numbers K and struggle with imbalanced graphs. We study deep graph clustering without K considering realistic imbalance through structural information theory. In the literature, structural information is rarely used in deep clustering, and its classic discrete definition neglects node attributes while exhibiting prohibitive complexity. In this paper, we establish a differentiable structural information framework, generalizing the discrete formalism to the continuous realm. We design a hyperbolic model (LSEnet) to learn the neural partitioning tree in the Lorentz model. Theoretically, we demonstrate its capability in clustering without K and identifying minority clusters. Second, we refine hyperbolic representations to enhance graph semantics. Since tree contrastive learning is non-trivial and costs quadratic complexity, we advance our theory by discovering that structural entropy bounds the tree contrastive loss. Finally, we approach graph clustering through a novel augmented structural information learning (ASIL), which offers an efficient objective to integrate hyperbolic partitioning tree construction and contrastive learning. With a provable improvement in graph conductance, ASIL achieves effective debiased graph clustering in linear complexity. Extensive experiments show ASIL outperforms 20 strong baselines by an average of +12.42% in NMI on the Citeseer dataset.

==> related.tex <==


\section{Related Work}

\textbf{Deep Graph Clustering.}
Deep models have achieved state-of-the-art results in node clustering.
Classic methods leverage a reconstructive loss to learn node representations, while identifying node clusters with distance-based or model-based algorithms (e.g., k-means, Gaussian mixture model) \cite{xie2016unsupervised,almahairi2016dynamic,yang2017graph}.
Other methods learn cluster assignment with generative adversarial nets \cite{DBLP:conf/ijcai/0002WGWCG20,DBLP:conf/www/JiaZ0W19}.
Contrastive clustering explores the similarity on the graph itself, pulling positive samples together and pushing negative ones apart \cite{devvrit2022s3gc,pan2021multi,DBLP:conf/www/LiJT22}. 
\cite{sun2023contrastive} consider contrastive graph clustering in the product manifold with a loss of Ricci curvature.
Normalizing flows have recently been introduced to graph clustering \cite{wang2023gc}.
%\citet{sun2023contrastive} introduce the geometric notion of curvature to deep clustering.
 Few deep model is  built without the predefined cluster number, to the best of our knowledge.
 Very recently, \cite{liu2023reinforcement} focus on automatically estimating the number of clusters via reinforcement learning, which is orthogonal to our study.
 %, and obtain clustering results with off-the-shelf algorithms (e.g., k-means)
 


\textbf{Structural Entropy.}
Information entropy is a key notation of information theory \cite{6773024}, measuring the amount of information for unstructured data, and it fails to study the information on graphs.
On information measure for graphs, early practices, e.g., Von Neumann entropy \cite{bra06} and Gibbs entropy \cite{bia09}, are still defined by unstructured probability distributions, and the graph structure is degenerated.
Recently, structural entropy is proposed in account of the natural self-organizing in the graphs \cite{li2016structural}, and has been successfully applied to graph pooling \cite{wu2022structural}, adversarial attack \cite{liu2019rem}, contrastive learning \cite{wu2023sega}, dimension estimation \cite{yang2023minimum} and graph structural learning \cite{zou2023segslb}. 
% We observe that the methods above are organized in a loose pipeline, i.e., structural entropy is first calculated  independently due to its discrete nature, and then the 
However, structural entropy has not yet been introduced to deep clustering, and the gap roots in the discrete formulation of \cite{li2016structural}.
Besides,  it falls short of considering node features that are important to graph clustering as well.

\textbf{Riemannian Graph Learning.}
Euclidean space has been the workhorse of graph learning for decades \cite{kdd14DeepWalk,kipf2017semisupervised,velickovic2018graph,DBLP:journals/pvldb/YeLC24}. 
In recent years, Riemannian manifolds have emerged as an exciting alternative.
Hyperbolic models \cite{nips17NickelK,chami2019hyperbolica,HVGNN,SunL22CIKM,SunL23AAAI,zhang2021lorentzian,icml18revisitHyperbolic,DBLP:conf/www/FuWSYWPL23} achieve remarkable success on the graphs   dominated by tree-like structures \cite{DBLP:journals/corr/abs-1006-5169}.
In fact, an arbitrary tree can be embedded in hyperbolic space with bounded distortion \cite{sarkar2012low}.
\cite{DBLP:conf/icdm/Fu0WSJWTPY21} study the optimal curvature of hyperbolic space for graph embedding.
Beyond hyperbolic space, the product manifolds \cite{aaai22SelfMix,SunL24AAAI} show its superiority on generic graph structures.
Recently, Ricci curvature of Riemannian geometry is given a differentiable surrogate for graph structural learning \cite{SunL23ICDM}.
Manifold vector fields (ordinary differential equations) \cite{SunL24WWW} are introduced to study information diffusion on the graphs \cite{SunL24SIGIR}.
Note that, \emph{the inherent connection between the tree and hyperbolic space supports the construction of our model,} \texttt{LSEnet}.
